Improving Large Language Models Function Calling and Interpretability via Guided-Structured Templates

Large language models (LLMs) have demonstrated strong reasoning and tool-use capabilities, yet they often fail in real-world tool-interactions due to incorrect parameterization, poor tool selection, or misinterpretation of user intent. These issues often stem from an incomplete understanding of user goals and inadequate comprehension of tool documentation. While Chain-of-Thought (CoT) prompting has proven effective for enhancing reasoning in general contexts, our analysis reveals that free-form CoT is insufficient and sometimes counterproductive for structured function-calling tasks. To address this, we introduce a curriculum-inspired framework that leverages structured reasoning templates to guide LLMs through more deliberate step-by-step instructions for generating function callings. Experimental results show that our method reduces tool-use errors, achieving 3-12% relative improvements over strong baselines across diverse model series and approaches. Moreover, our framework enhances the robustness, interpretability, and transparency of tool-using agents, advancing the development of more reliable AI assistants for real-world applications.

==> latex/4_experiment_old.tex <==
\section{Experimental Details} \label{sec:experiments_results}

We conducted experiments to assess the effectiveness of internalizing structured reasoning into language models using our detailed templates. The evaluation focused on two standard benchmarks, BFCL (v1 and v2) and Nexus, both of which comprehensively measure function-calling capabilities across scenarios of varying complexity (e.g., simple, parallel, multi-parameter function calls).
\subsection{Template-Based Reasoning via Prompting}

We first compared three distinct prompting strategies to investigate the benefits of structured, template-based reasoning:

\begin{enumerate} \item \textbf{Direct Generation (Baseline):} The model directly produces the function call without generating intermediate reasoning steps. \item \textbf{Chain-of-Thought (CoT) Prompting:} A standard CoT prompt instructing the model to “Think step by step,” enabling free-form intermediate reasoning. \item \textbf{Template-Based Prompting (Our method):} A structured prompt following explicit templates, enforcing detailed intermediate reasoning steps as outlined in Section~\ref{subsec:prompting_strategies}. \end{enumerate}

We evaluate diverse language models including both closed-source and open-source from different models' group and sizes under these strategies including:

GPT-4o-FC, GPT-4o-mini-FC (closed-source, optimized for direct function calling, does not explicitly generate reasoning). For "FC" models, structured templates were embedded directly into the prompt without the requirement of explicitly outputting internal thoughts.

GPT-4o-mini-Prompting (closed-source, but enabling thinking before generations, after some preliminary experiments, GPT-4o-Prompting approaches struggle with format issues, which affect evaluation thus we do not report this model in experiments
Open-Source models including Llama-3.1-8B-Instruct, Mistral-7B-Instruct-v0.3, Mistral-Nemo-12B and Qwen-2.5-14B-Instruct (open-source, capable of explicitly generating intermediate reasoning). For these model(s), the model explicitly generated intermediate reasoning, guided by either CoT or our structured template prompts.
% Detailed experimental prompts and comprehensive sub-scores per test category are provided in Appendix Table1a (weighted average scores) and Table1b (sub-category breakdown).

\paragraph{Intermediate Reasoning via Templates Benefits Smaller Models.}


\paragraph{Template-Based Reasoning Outperforms Free-form CoT.}

A summary of these results is presented in Table~\ref{table:bfcl_short}.
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Prompting Method}} 
 & \textbf{BFCL-v2 Benchmark} & \textbf{Nexus Benchmark} \\
  & & \textbf{Weighted / BFCL Average} & \textbf{Weighted / Unweighted Average} \\
\midrule
\multicolumn{4}{l}{\textbf{Function Calling Generation Only}} \\
\midrule
\multirow{3}{*}{GPT-4o-FC}
 & No Thought & 73.78 / 74.79 & – / – \\
 & CoT Prompting & 77.40 / 78.83 & – / – \\
 & Template-Based Prompting & \textbf{78.99} / \textbf{80.26} & – / – \\
\midrule
\multirow{3}{*}{GPT-4o-mini-FC}
 & No Thought & 73.52 / 74.72 & – / – \\
 & CoT Prompting & 77.34 / 78.71 & – / – \\
 & Template-Based Prompting & \textbf{78.30} / \textbf{79.79} & – / – \\
\midrule
\multicolumn{4}{l}{\textbf{Function Calling and Thought Generation}} \\
\midrule
\multirow{3}{*}{GPT-4o-mini Prompting}
 & No Thought & 78.99 / 80.25 & 36.85 / 34.01 \\
 & CoT Prompting & \textbf{79.87} / \textbf{80.59} & 40.61 / 35.26 \\
 & Template-Based Prompting & 79.70 / 80.24 & \textbf{41.33} / \textbf{36.20} \\
\midrule
\multirow{3}{*}{LLaMA-3.1-8B-Instruct}
 & No Thought & 64.43 / 65.75 & 35.40 / 30.06 \\
 & CoT Prompting & 65.28 / 66.70 & 36.71 / 30.06 \\
 & Template-Based Prompting & \textbf{68.28} / \textbf{69.65} & \textbf{38.01} / \textbf{33.09} \\
\midrule
\multirow{3}{*}{Mistral-7B-Instruct-v0.3}
 & No Thought & \textbf{60.70 / 57.55} & 10.84 / 9.05 \\
 & CoT Prompting & 51.11 / 48.94 & \textbf{26.01 / 22.26} \\
 & Template-Based Prompting & 48.83 / 46.88 & 25.29 / 20.80 \\
\midrule
\multirow{3}{*}{Mistral-Nemo-12B}
 & No Thought & 57.92 / 58.90 & 25.72 / 22.08 \\
 & CoT Prompting & 63.31 / 65.19 & 31.50 / 27.78 \\
 & Template-Based Prompting & \textbf{64.71} / \textbf{66.32} & \textbf{32.95} / \textbf{28.46} \\
\midrule
\multirow{3}{*}{Qwen-2.5-14B-Instruct}
 & No Thought & \textbf{76.22 / 77.33} & 43.21 / 38.57 \\
 & CoT Prompting & 68.06 / 62.25 & 41.33 / 35.38 \\
 & Template-Based Prompting & 74.37 / 73.28 & \textbf{44.07} / \textbf{40.78} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison across BFCL-v2 and Nexus Function Calling benchmarks. Bold values indicate the highest scores within each model group.}
\label{tab:bfcl_nexus_results}
\end{table*}

\subsection{Fine-Tuning with Structured Reasoning}
% \hdcomment{Add Training Hyperparameters and settings}
To further investigate the effect of explicitly internalizing structured reasoning within model parameters, we performed supervised fine-tuning (SFT) experiments utilizing the constructed data set described in Section~\ref{subsec:sft_data_construction}. The following training strategies were evaluated:
\begin{itemize}
    \item \textbf{No Thought}: We trained baseline models exclusively on final function-call tokens, deliberately omitting intermediate reasoning steps. This baseline replicates common practices in existing function call literature, optimizing solely for the final prediction.
    \item \textbf{CoT-Training}: As discussed, we additionally evaluate if models' own thinking reasoning could help in function calling's capabilities. Thus, we follow our training data generations steps but instead of template-based reasoning, we encourage models to generate their own reasonings to support function calling(s).
    \item \textbf{Template-Training}: In contrast, we explicitly include intermediate structured reasoning steps following our templates within the training data. Models optimized a combined cross-entropy loss on both intermediate reasoning and final function call tokens, internalizing the structured reasoning methodology explicitly into their parameters.
\end{itemize}
We evaluated the performance improvements across three open-source architectures: Llama-3.1-Instruct (8B), Mistral-Instruct (7B, 12B), and Qwen-2.5-Instruct (14B). Our key findings are summarized below.

\paragraph{Structured Reasoning via SFT Improves Function-Calling Robustness.}
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Dataset}} 
 & \textbf{BFCL-v2 Benchmark} & \textbf{Nexus Benchmark} \\
  & & \textbf{Weighted / BFCL Average} & \textbf{Weighted / Unweighted Average} \\
\midrule
\multirow{3}{*}{LLaMA-3.1-8B-Instruct}
 & No Thought & 69.73 / 72.16 & 35.98 / 29.82 \\
 & CoT-Training & 73.33 / 74.74 & \textbf{36.85} / 30.19 \\
 & Template-Training & \textbf{74.10} / \textbf{75.28} & 36.27 / \textbf{30.23} \\
\midrule
\multirow{3}{*}{Mistral-7B-Instruct-v0.3}
 & No Thought & 64.65 / 66.51 & 26.59 / 21.78 \\
 & CoT-Training & 67.06 / 69.16 & 24.85 / 20.55 \\
 & Template-Training & \textbf{69.87} / \textbf{71.40} & \textbf{27.02} / \textbf{23.17} \\
\midrule
\multirow{3}{*}{Mistral-Nemo-12B}
 & No Thought & 74.87 / 76.44 & 32.66 / 26.46 \\
 & CoT-Training & 76.60 / 77.72 & 35.69 / 31.00 \\
 & Template-Training & \textbf{77.40} / \textbf{78.63} & \textbf{37.28} / \textbf{32.46} \\
\midrule
\multirow{3}{*}{Qwen-2.5-14B-Instruct}
 & No Thought & 77.06 / 78.61 & 40.74 / 35.72 \\
 & CoT-Training & 77.92 / 79.46 & 40.75 / 35.85 \\
 & Template-Training & \textbf{78.55} / \textbf{79.83} & \textbf{42.20} / \textbf{37.05} \\
\bottomrule
\end{tabular}
}
\caption{Results on BFCL-v2 and Nexus Function Calling using SFT-ed models with prompts trained on Baseline, CoT, or Template data. Bold values indicate the best score for each model.}
\label{tab:sft_bfcl_nexus}
\end{table*}
\subsubsection{Ablation Studies}
\subsection{Impact of Template Complexity on Performance} \label{subsec:template_ablation}

To better understand how the structure and specificity of reasoning templates influence function-calling performance, we conducted additional ablation experiments comparing three distinct prompting templates: \emph{Simple}, \emph{Claude}, and \emph{Detail}. The detailed specifications of the reasoning templates used in our experiments are provided in Table~\ref{table:templates_details} in the Appendix.

Our results, summarized in Table~\ref{table:bfcl_template_ablation}, show that templates incorporating more explicit, stepwise reasoning generally lead to superior overall accuracy. For instance, the \emph{Detail} template outperforms other templates consistently: \textbf{Mistral-v0.3-Instruct} achieves a 69.87 weighted average score with the Detail template, compared to 68.63 (Simple) and 60.64 (Claude). Similarly, \textbf{Llama-3.1-8B-Instruct} records an overall score of 74.10 with the Detail template, compared to 71.27 (Simple) and 70.20 (Claude).

However, our analysis also revealed that simpler templates occasionally outperform detailed ones on specific subtasks, such as \textit{Relevance/Irrelevance}. This observation highlights an important direction for future work: adopting a \textbf{dynamic prompting approach}, in which models adapt their reasoning granularity based on the complexity and type of the user's query, potentially combining the advantages of different template styles.
\begin{table*}[htbp]
    
    \centering
    \caption{Ablation study comparing performance across different prompting templates (Simple, Claude, and Detail) to generate training data including without (No Thought) and with explicit intermediate reasoning ("Thought"). No Thought version includes same training samples as Thought version except without reasoning step provided but rather direct finetuning with ground truth function calling(s). Evaluation is based on the BFCL benchmark using weighted average metric.}
    \label{table:bfcl_template_ablation}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llcccccc}
        \toprule
        & & \multicolumn{3}{c}{\textbf{Llama-3.1-8B-Instruct}} & \multicolumn{3}{c}{\textbf{Mistral-v0.3-Instruct}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        \textbf{Category} & \textbf{Training Data} & \textbf{Simple} & \textbf{Claude} & \textbf{Detail} & \textbf{Simple} & \textbf{Claude} & \textbf{Detail} \\
        \midrule
        \multirow{2}{*}{Overall Score} 
        & No Thought & 64.49 & 61.55 & 62.76 & 66.44 & 47.73 & 64.65 \\
        & Thought & 71.27 & 70.20 & \textbf{74.10} & 68.63 & 60.64 & \textbf{69.87} \\
        \midrule
        % \multirow{2}{*}{Non-Live Average} 
        % & No Thought & \textbf{86.96} & \textbf{86.96} & 84.70 & \textbf{83.74} & 74.61 & 83.39 \\
        Non-Live Average & Thought & 80.43 & 79.57 & \textbf{84.61} & 78.52 & 70.26 & \textbf{81.22} \\
        \midrule
        % \multirow{2}{*}{Live Average} 
        % & No Thought & \textbf{63.37} & 61.65 & 59.40 & 64.20 & 47.34 & \textbf{64.27} \\
        Live Average & Thought & 55.58 & 54.60 & \textbf{63.68} & 55.35 & 47.19 & \textbf{59.92} \\
        \midrule
        % \multirow{2}{*}{Relevance/Irrelevance} 
        % & No Thought & 43.43 & 36.16 & \textbf{44.81}& \textbf{51.82} & 21.45 & 46.45 \\
        Relevance/Irrelevance & Thought & \textbf{80.28} & 78.90 & 75.61 & \textbf{74.13} & 66.59 & 70.07 \\
        \bottomrule
    \end{tabular}}
\end{table*}

% \paragraph{Dynamic Reasoning Analysis}

